Beyond Ideological Similarity: Theme and Tone Supervision for Political Text Classification

Political-text classifiers support research on ideology, stance, and media bias, yet a high average score can hide errors that reverse a position or systematically erase and attribute bias. We test whether supervision from semantic themes and net evaluative tone changes a RoBERTa representation trained with ideology triplet loss and masked language modeling. Across facet-level ideology, sentence-level media bias, and target-conditioned stance, no auxiliary objective dominates. Instead, theme, tone, and joint supervision help different tasks and alter different error directions. For example, joint supervision lowers lexical-bias erasure at The New York Times from 52.7% to 36.9%, but raises Against-to-Favor stance reversals from 12.8% to 15.2%. These effects change when auxiliary labels cover only part of the pre-training corpus. Metalinguistic supervision is therefore a design choice, not a universal upgrade: researchers should test which signal matches the construct and error costs of the intended analysis.

==> sections/future_work.tex <==
\section{Future Work}
\label{sec:future-work}
\flag{S8 del: whole section removed; see Conclusion}
% Our findings demonstrate that metalinguistic objectives improve article-level ideology classification, though several methodological constraints limit the scope of the current investigation.
Our findings demonstrate that metalinguistic objectives can improve political-text classification in specific settings, though several methodological constraints limit the scope of the current investigation.

A first priority is broadening and diversifying metalinguistic supervision. This includes increasing GDELT coverage or sourcing alternative annotations to raise the proportion of supervised articles, and expanding the auxiliary feature set beyond theme and tone to include sentiment intensity, subjectivity, emotional valence, and discourse markers. Combining heterogeneous metalinguistic signals may enable richer representations of ideological framing, and examining transferability across transformer architectures and model sizes would clarify the generality of the approach.

Additionally, integrating explainability techniques with metalinguistic pre-training could enhance model interpretability, enabling researchers and practitioners to understand how specific linguistic cues influence ideology predictions.


==> tables/table_outlet_gap.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{3.2pt}
\begin{tabular}{@{}lrrr@{}}
\toprule
Model & Fox & NYT & Gap \\
\midrule
RoBERTa & $57.2$ & $39.2$ & $+18.0$ \\
$MLM+T_{id}(16)$ & $51.6$ & $52.7$ & $\mathbf{-1.1}$ \\
$+T_h$ & $51.6$ & $44.2$ & $+7.4$ \\
$+T_o$ & $51.2$ & $42.7$ & $+8.5$ \\
$+T_h+T_o$ & $\mathbf{45.4}$ & $\mathbf{36.9}$ & $+8.5$ \\
\bottomrule
\end{tabular}
\caption{Dense-subset lexical-bias erasure at Fox News and \textit{The New York Times}, in percent. Joint supervision lowers erasure at both outlets, but by 6.2 points at Fox and 15.8 at the \textit{Times}. The gap is Fox minus NYT; zero indicates equal erasure.}
\label{tab:outlet-gap}
\end{table}

